EntGPT: Entity Linking with Generative Large Language Models

Entity Linking in natural language processing seeks to match text entities to their corresponding entries in a dictionary or knowledge base. Traditional approaches rely on contextual models, which can be complex, hard to train, and have limited transferability across different domains. Generative large language models like GPT offer a promising alternative but often underperform with naive prompts. In this study, we introduce EntGPT, employing advanced prompt engineering to enhance EL tasks. Our three-step hard-prompting method (EntGPT-P) significantly boosts the micro-F_1 score by up to 36% over vanilla prompts, achieving competitive performance across 10 datasets without supervised fine-tuning. Additionally, our instruction tuning method (EntGPT-I) improves micro-F_1 scores by 2.1% on average in supervised EL tasks and outperforms several baseline models in six Question Answering tasks. Our methods are compatible with both open-source and proprietary LLMs. All data and code are available on GitHub at https://github.com/yifding/In_Context_EL.

==> table/dataset_stats.tex <==
% \resizebox{\textwidth}{!}{%
%\begin{tabular}{l | ccccccccccc}
%\toprule 
% & \textbf{AIDA} & \textbf{MSN} & \textbf{AQU} & \textbf{ACE04}
% & \textbf{CWEB} & \textbf{WIKI} &
% \textbf{KORE} & 
% \textbf{OKE15} & \textbf{OKE16} &
%\textbf{REU} & \textbf{RSS}   \\
%\midrule
%\# of Docs & 231 & 20 & 50 & 35 & 320 & 319 & 50 & 101 & 173 & 113 & 357 \\
%\# of Mention & 4485 & 656 & 727 & 257 & 11154 & 6793 & 144 & 536 & 288 & 650 & 524\\
%\bottomrule
%\end{tabular}


\begin{tabular}{l | c c}
\toprule
 & \textbf{\# of Docs} & \textbf{\# of Mentions} \\
\midrule
\textbf{AIDA} & 231 & 4485 \\
\textbf{MSN} & 20 & 656 \\
\textbf{AQU} & 50 & 727 \\
\textbf{ACE04} & 35 & 257 \\
\textbf{CWEB} & 320 & 11154 \\
\textbf{WIKI} & 319 & 6793 \\
\textbf{KORE} & 50 & 144 \\
\textbf{OKE15} & 101 & 536 \\
\textbf{OKE16} & 173 & 288 \\
\textbf{REU} & 113 & 650 \\
\textbf{RSS} & 357 & 524 \\
\bottomrule
\end{tabular}


% \begin{tabular}{l|ccccc}
%     \toprule 
%     Out-of-domain & \textbf{KORE} & \textbf{OKE15} & \textbf{OKE16} &\textbf{REU} & \textbf{RSS} \\ \midrule
%     \# of Docs & 50	& 101	& 173	& 113	& 357 \\
%     \# of Mention &144	&536	&288	&650	&524 \\
%     \toprule
%     In-domain & \textbf{ACE04} &
%     \textbf{MSN} & \textbf{WIKI} & \textbf{AQU} & \textbf{CWEB}\\
%     \# of Docs &35	&20	&319 &50 &320 \\ \midrule
%     \# of Mention &257	&656	&6793	&727	&11154 \\
%     \bottomrule
% \end{tabular}

==> table/error_case_study.tex <==
%\resizebox{\textwidth}{!}{%
%{
\begin{tabular}{ccccc}
\toprule
Dataset & Degree of Error & Ground Truth & Prediction & Reason Analysis \\
ACE04	&high	&Ministry of Defense (Iran)	&Ministry of Defense (Japan)	&2nd prompt  \\
ACE04	&high	&Florida	&Florida Legislature	&2nd prompt \\
ACE04	&low	&President of Egypt	&President	&2nd prompt \\
ACE04	&low	&Gaza City	&Gaza Strip	&1st prompt \\
ACE04	&low	&Volvo	&Volvo Cars	&2nd prompt    \\
KORE	&low	&First Ladies of Argentina	&First Lady	&1st prompt \\
KORE	&high	&Justin Bieber	&Justin I	&1st prompt \\
KORE	&high	&Lady Gaga	&Gwen Stefani	&2nd prompt \\
KORE	&high	&Desire (Bob Dylan album)	&Desire	&post-processing \\
KORE	&high	&Paul Allen	&NULL	&1st prompt \\
AQU	&high	&Cancer	&Lung Cancer	&2nd prompt \\
AQU	&high	&Tissue (biology)	&Facial tissue	&2nd prompt \\
AQU	&high	&Radiation	&Ionizing Radiation	&2nd prompt \\
AQU	&high	&Federation	&Malaysian Roads System	&1st prompt \\
AQU	&high	&Federated State	&States of India	&2nd prompt \\
CWEB	&high	&Head	&Head (company)	&1st prompt \\
CWEB	&-	&Hillsborough County, Florida	&Hillsborough, North Carolina	&GT is incorrect \\
CWEB	&low	&Lake Wylie	&Lake Wylie, South Carolina	&2nd prompt \\
CWEB	&-	&Australia Cricket Team	&Australia	&GT is incorrect \\
CWEB	&high	&England Cricket Board	&European Central Bank	&2nd prompt \\
MSN	&high	&Associated Press	&Arnold Ap	&2nd prompt \\
MSN	&-	&New York City	&New York	&GT is incorrect \\
MSN	&-	&University of Alabama	&Alabama Crimson Tide football	&GT is incorrect \\
MSN	&high	&Sago Mine Disaster	&Sago, West Virginia	&1st prompt \\
MSN	&high	&World Trade Center	&Collapse of the World Trade Center	&2nd prompt \\
OKE15	&-	&Fellow	&Research Fellow	&GT is incorrect \\
OKE15	&low	&Cambridge	&University of Cambridge	&1st prompt \\
OKE15	&-	&Principal (academia)	&Head teacher	&GT is incorrect \\
OKE15	&low	&Faculty (academic staff)	&Professor	&1st prompt \\
OKE15	&-	&Officer	&Officer (armed forces)	&GT is incorrect \\
OKE16	&-	&Director (business)	&Executive director	&GT is incorrect \\
OKE16	&-	&Germany	&Nazi Germany	&GT is incorrect \\
OKE16	&-	&Czechs	&Czech Republic	&GT is incorrect \\
OKE16	&high	&Salvatore Quasimodo	&Quasimodo	&1st prompt \\
OKE16	&-	&Sorbonne	&University of Paris	&GT is incorrect \\
REU	&high	&Oregon	&Ore	&post-processing \\
REU	&-	&Georgia Power	&Georgia (U.S. state)	&GT is incorrect \\
REU	&low	&Lloyds Bank of Canada	&Lloyds Bank	&2nd prompt \\
REU	&high	&Continental Bank of Canada	&Continental philosophy	&1st prompt \\
REU	&high	&J. P. Morgan	&Morgan Motor Company	&1st prompt \\
RSS	&-	&Steve Jobs	&Apple Inc.	&GT is incorrect \\
RSS	&low	&Pro Bowl	&Super Bowl	&2nd prompt \\
RSS	&high	&Pro Bowl	&Bowl Game	&2nd prompt \\
RSS	&-	&Eric Kearney	&Cincinnati	&GT is incorrect \\
RSS	&high	&Cleveland Browns	&Cleveland	&2nd prompt \\
WIKI &low	&Croatia Speedway Team	&Croatia	&2nd prompt \\
WIKI	&low	&Little Caesars Pizza Bowl	&2009 Little Caesars Pizza Bowl	&prediction is better \\
WIKI	&low	&Ohio Bobcats football	&Ohio Bobcats	&2nd prompt \\
WIKI	&low	&Leasehold estate	&Renting	& 1st prompt \\
WIKI	&low	&Real Estate Pricing	&House Price Index	&2nd prompt \\

\bottomrule
\end{tabular}
%}
%}



==> table/error_type.tex <==
%\resizebox{\textwidth}{!}{%
%{
\begin{tabular}{rl | ccccc | ccccc }
\toprule
&\multirow{2}{*}{\textbf{Error Type}} & \multicolumn{5}{c|}{\textbf{Out-of-domain}} & \multicolumn{5}{c}{\textbf{In-domain}} \\

& & \textbf{KORE} & \textbf{OKE15} & \textbf{OKE16} &
\textbf{REU} & \textbf{RSS} & \textbf{ACE04} &
\textbf{MSN} & \textbf{WIKI} & \textbf{AQU} & \textbf{CWEB} \\

\midrule
\multirow{2}{*}{\textbf{FP}} & \textbf{Alternative Entity} &4	&26	&27	&34	&12	&11	&34	&507	&71	&1318 \\
& \textbf{Fail to Reject} &8	&17	&19	&47	&42	&7	&2	&402	&12	&440\\
\midrule
\multirow{2}{*}{\textbf{FN}} & \textbf{Miss GT} &8	&62	&63	&34	&32	&9	&38	&535	&125	&1558\\
& \textbf{Miss Candidate} &23	&78	&76	&59	&35	&8	&37	&315	&15	&753\\


\bottomrule
\end{tabular}
%}
%}


